Transformers as Algorithms: Generalization and Stability in In-context Learning

In-context learning (ICL) is a type of prompting where a transformer model operates on a sequence of (input, output) examples and performs inference on-the-fly. In this work, we formalize in-context learning as an algorithm learning problem where a transformer model implicitly constructs a hypothesis function at inference-time. We first explore the statistical aspects of this abstraction through the lens of multitask learning: We obtain generalization bounds for ICL when the input prompt is (1) a sequence of i.i.d. (input, label) pairs or (2) a trajectory arising from a dynamical system. The crux of our analysis is relating the excess risk to the stability of the algorithm implemented by the transformer. We characterize when transformer/attention architecture provably obeys the stability condition and also provide empirical verification. For generalization on unseen tasks, we identify an inductive bias phenomenon in which the transfer learning risk is governed by the task complexity and the number of MTL tasks in a highly predictable manner. Finally, we provide numerical evaluations that (1) demonstrate transformers can indeed implement near-optimal algorithms on classical regression problems with i.i.d. and dynamic data, (2) provide insights on stability, and (3) verify our theoretical predictions.

==> app/lemma.tex <==
\section{Useful lemmas}


==> app/mtl_proof.tex <==
\section{Proof of Theorem~\ref{thm mtl}}
% \begin{definition}[Data-dependent distance metric $\rho$]\label{def:distance metric} 
%     Let $\Qc:\Xc\rightarrow\R^r$ be a family of functions. Given $q,q'\in\Qc$ and an input dataset $\X=\{\x_1,\dots,\x_n\}$ with $\x_i\in\Xc$, we define the dataset-dependent Euclidean distance by $\rho_\X(q,q'):=\sqrt{\frac{1}{n}\sum_{i\in[n],j\in[r]}(q_j(\x_i)-q'_j(\x_i))^2}=\sqrt{\frac{1}{n}\sum_{i\in[n]}\tn{q(\x_i)-q'(\x_i)}^2}$, where $q(\x)=[q_1(\x),\dots,q_r(\x)]^\top$.
% \end{definition}
\begin{definition}[Gaussian complexity of $\Ac$]\label{def rad} Let $\Ac:\Zc\rightarrow\R$ be a set of algorithm hypotheses. Let $((g_{ti})_{i=1}^{n})_{t=1}^T\in\R$ be $nT$ independent normal random variables. Then given dataset $\Sca=\{\Sc_t\}_{t=1}^T$ where $\Sc_t=\{(\x_{ti},y_{ti})\}_{i=1}^n$, the empirical Gaussian complexity is defined as 
	\[
		\Gch_\Sca(\Ac)=\E_{g_{ti}}\left[\sup_{\bal\in\Ac}\frac{1}{nT}\sum_{t=1}^T\sum_{i=1}^ng_{ti}\fal{i-1}{t}(\x_{ti})\right].
	\]
The worst-case Gaussian complexity is obtained by considering the supremum over all $\Sca$ as follows.
	\[
		\Gct_{nT}(\Ac)=\sup_{\Sca}\left[\Gch_\Sca(\Ac)\right].
	\]
\end{definition}
\begin{definition}[Covering number ]\label{def cover} Let $\Ac:\Zc\rightarrow\R$ be a set of algorithm hypotheses. Given $\bal,\bal'\in\Ac$, and a distance metric $d(\bal,\bal')\geq0$, $\Ac_\eps=\{\bal_1,\dots,\bal_N\}$ is the $\eps$-cover of $\Ac$ with respect to the distance metric $d$ if for any $\bal\in\Ac$, there exists $\bal_i\in\Ac_\eps$ such that $d(\bal,\bal_i)\leq\eps$. Define the cardinality of the minimal $\eps$-covers as $\eps$-covering number defined by $\Nc(\Ac,d;\eps)$.  
\end{definition}
\begin{definition}[Data-dependent distance metric over $\Ac$]\label{def distance} Let $\Ac:\Zc\rightarrow\R$ be a set of algorithm hypotheses. Assume there are $T$ tasks $\{\Sc_t\}_{t}^T$ where $\Sc_t=\{(\x_{ti},y_{ti})\}_{i=1}^n$. Following \eqref{mtl opt}, given any $\bal\in\Ac$, let $\yal=((\fal{i-1}{t}(\x_{ti}))_{i=1}^n)_{t=1}^T$. Then we define the distance metric of $\Ac$ over $\Sca$ by $\rho_\Sca(\bal,\bal'):=\|\yal-\yalp\|$.
\end{definition}
% \begin{definition}[Distance metric over $\Ac$]\label{def distance} Let $\Ac:\Zc\rightarrow\R$ be a set of algorithm hypotheses. Assume there are $T$ tasks $\Sca:=\bigcup_{t=1}^T\Sc_t$ where $\Sc_t=\{(\x_{ti},y_{ti})\}_{i=1}^n\sim\Dc_t$. Let $\Dca=\{\Dc_t\}_{t=1}^T$. Given any $\bal\in\Ac$, let $\yal=((\fal{i-1}{t}(\x_{ti}))_{i=1}^n)_{t=1}^T$. Then we define the distance metric of $\Ac$ by $\rho(\bal,\bal'):=\sup_{\Sca\sim\Dca}\|\yal-\yalp\|$.
% \end{definition}
% \begin{theorem} [Theorem~\ref{thm mtl} restated]
% Assume loss function $\ell(y,\hat y)$ takes values in $[0,B]$ and is an $L$-Lipschitz function. 
% %    Any $\fal{i-1}{t}$ generated by $\bal$ and $\Scnt{i-1}{t}\distas\Dc_t$ is a $\Gamma$-Lipschitz function.
% Let $\bah$ be the empirical solution of \eqref{mtl opt}. Then with probability at least $1-2e^{-\tau}$, the excess test risk $\Rmtl(\bah)$ obeys
% \[
% 	\Rmtl(\bah)\leq
% \]
% \end{theorem}
\begin{proof}
Recap the MTL problem that assume there are $T$ contexts each with $n$ training samples denoted by $(\Sc_t)_{t=1}^T\distas(\Dc_t)_{t=1}^T$ where $\Sc_t=\{(x_{ti},y_{ti})\}_{i=1}^n$. Let $\bal^\st=\arg\min_{\bal\in\Ac}\Lc_\Dca(\bal)$ and $\bah=\arg\min_{\bal\in\Ac}\Lch_\Sca(\bal)$ where $\Lch_\Sca(\bal)=\frac{1}{nT}\sum_{t=1}^{T}\sum_{i=1}^n\ell(y_{ti},\fal{i-1}{t}(\x_{ti}))$ and $\Lc_\Dca(\bal)=\E[\Lch_\Sca(\bal)]$. Then following Eq.~\eqref{mtl risk}, we have the MTL excess test risk
\begin{align}
    \Rmtl(\bah)=\underset{\text{generalization error} (\Rgen)}{\underbrace{\Lc_\Dca(\bah)-\Lc_\Dca(\bal^\st)}} + \underset{\text{approximation error}(\Rapx)}{\underbrace{\Lc_\Dca(\bal^\st) - \Lc^\st_{\f}}}.
\end{align}
We will start with bounding the generalization error ($\Rgen(\bah)$), where we have
\begin{align}
	\Rgen&=\Lc_\Dca(\bah)-\Lc_\Dca(\bal^\st)\\
	&=\underset{a}{\underbrace{\Lc_\Dca(\bah)-\Lch_\Sca(\bah)}}+\underset{b}{\underbrace{\Lch_\Sca(\bah)-\Lch_\Sca(\bal^\st)}}+\underset{c}{\underbrace{\Lch_\Sca(\bal^\st)-\Lc_\Dca(\bal^\st)}}.
\end{align}
Since $\bah$ is the minimizer of empirical risk, intuitively we have $b\leq0$. In the following, we consider the concentration problem that for any $\bal\in\Ac$, how to upper bound $|\Lc_\Dca(\bal)-\Lch_\Sca(\bal)|$. For cleaner notations, in the following we drop the subscripts $\Dca$ and $\Sca$.

\textbf{Step 1: We start with the concentration bounds based on the discrete search space.} Let $\bAc$ be a discrete algorithm hypothesis set where $\bAc\subset\Ac$. Denote the cardinality of $\bAc$ by $|\bAc|=D$. We are interested in the problem that given any $\bal\in\bAc$, how $|\Lc(\bal)-\Lch(\bal)|$ can be bounded.
% Following Definition~\ref{def cover}\&\ref{def distance}, let $\Ac_\eps$ be $\eps$-cover of $\Ac$ based on distance metric $\rho_\Sca(\cdot,\cdot)$ and $\Nc(\Ac,\rho_\Sca;\eps)$ is the covering number. 
%Define $\Lch_t(\bal)=\sum_{i=1}^n\ell(y_{ti},\fal{i-1}{t}(\x_{ti}))$ and $\Lc_t(\bal)=\E[\Lch_t(\bal)]$. Then we have that $\Lch=\frac{1}{T}\sum_{t=1}^T{\Lch_t}$ and $\Lc=\frac{1}{T}\sum_{t=1}^T\Lc_t$. 

Define the random variables $X_{ti}=\E[\Lch(\bal)|\Sc_1,\dots,\Sc_{t-1},\Scnt{i}{t}]$, that is, $X_{ti}$ is the expectation over $\Lch(\bal)$ given training data of $\Sc_1,\dots,\Sc_{t-1}$ datasets (each with $n$ samples) and $i$ samples from $t$'th context. Then we get sequence $\{X_{1,0},X_{1,1}\dots,X_{1,n},X_{2,1}\dots,X_{2,n}\dots ,X_{T,1}\dots,X_{T,n}\}$ where we $X_{1,0}=\E[\Lch(\bal)]=\Lc(\bal)$, $X_{T,n}=\E[\Lch(\bal)|\Sc_1,\dots,\Sc_T]=\Lch(\bal)$ and $\E[X_{ti}]=\Lc(\bal)=X_{1,0}$. Therefore, $\{X_{1,0}\dots,X_{T,n}\}$ is a Martingale sequence, and we have \red{$|X_{ti}-X_{t,i-1}|,|X_{t,1}-X_{t-1,n}|\leq B'/nT$}. Applying Azuma-Hoeffding's inequality, we can obtain
\begin{align}
    \P\left(|X_{T,n}-X_{1,0}|\geq t\right)\leq2 e^{-\frac{nTt^2}{2B'^2}}\Longrightarrow\P(|\Lch-\Lc|\geq t)\leq2 e^{-\frac{nTt^2}{2B'^2}}.
\end{align}
Applying union bound over $\bAc$ and setting $t=2B'\sqrt{\frac{\log D+\tau}{nT}}$, we have that for any $\bal\in\bAc$, with probability at least $1-2e^{-\tau}$,
\[
	|\Lch(\bal)-\Lc(\bal)|\leq2B'\sqrt{\frac{\log D+\tau}{nT}}.
\]

\textbf{Step 1: We start with the concentration bounds based on the discrete search space. (Emrullah)} Let $\bAc$ be a discrete algorithm hypothesis set where $\bAc\subset\Ac$. Denote the cardinality of $\bAc$ by $|\bAc|=D$. We are interested in the problem that given any $\bal\in\bAc$, how $|\Lc(\bal)-\Lch(\bal)|$ can be bounded.
% Following Definition~\ref{def cover}\&\ref{def distance}, let $\Ac_\eps$ be $\eps$-cover of $\Ac$ based on distance metric $\rho_\Sca(\cdot,\cdot)$ and $\Nc(\Ac,\rho_\Sca;\eps)$ is the covering number. 
%Define $\Lch_t(\bal)=\sum_{i=1}^n\ell(y_{ti},\fal{i-1}{t}(\x_{ti}))$ and $\Lc_t(\bal)=\E[\Lch_t(\bal)]$. Then we have that $\Lch=\frac{1}{T}\sum_{t=1}^T{\Lch_t}$ and $\Lc=\frac{1}{T}\sum_{t=1}^T\Lc_t$. 
Let us define the loss for each task separately:
\begin{align}
	&\Lch_t(\bal) :=\frac{1}{n}\sum_{i=1}^n \ell(y_{ti},\fal{i-1}{t}(\x_{ti})) \quad \forall t \in [T] \nonumber \\
	&\Lc_t(\bal) :=\frac{1}{n}\sum_{i=1}^n \E[\ell(y_{ti},\fal{i-1}{t}(\x_{ti}))] \quad \forall t \in [T] \nonumber
\end{align}
Define the random variables $X_{t,i}=\E[\Lch_t(\bal)|\Scnt{i}{t}]$ for $i \in [n]$ and $t \in [T]$, that is, $X_{ti}$ is the expectation over $\Lch(\bal)$ given training data of $\Scnt{i}{t}=\{(\x_j^{(t)},y_j^{(t)})\}_{j=1}^i$. Let $X_{t,0} = \E[\Lch_t(\bal)]$ for $t \in [T]$. Then, for every $t$ in $[T]$, the sequences $\{X_{t,0}, X_{t,1}, 
\dots, X_{t,n}\}$ are Martingale sequences with respect to $\Scnt{i}{t}$:
\begin{align}
	&\E[X_{t,i}] \leq B < \infty \nonumber \\
	&\E[X_{t,i+1} | \Scnt{i}{t}] = X_{t,i} \nonumber
\end{align}
\begin{comment}

Let's look at the difference: (for the sake of simplicity in the notation, we omit the subscript $t$)
\begin{align}
	|X_{t,i} - X_{t,i-1}| &= \E\bigg[\frac{1}{n}\sum_{i=1}^n \ell(y_{i},\fal{i-1}{}(\x_{i})) \bigg| \Scnt{i}{}\bigg] - \E\bigg[\frac{1}{n}\sum_{i=1}^n \ell(y_{i},\fal{i-1}{}(\x_{i})) \bigg| \Scnt{i-1}{}\bigg]\nonumber \\
	&= \frac{1}{n}\sum_{j=i}^n \E[\ell (y_j, \fal{i}{}(x_j)) | \Scnt{i}{}] - \E[\ell(y_j, \fal{i-1}{}(x_j))| \Scnt{i-1}{}] \nonumber \\
	&\leq \frac{B}{n} + \frac{1}{n}\sum_{j=i+1}^n \E[\ell (y_j, \fal{i}{}(x_j)) | \Scnt{i}{}] - \E[\ell(y_j, \fal{i-1}{}(x_j))| \Scnt{i-1}{}] \nonumber \\
	& \hspace{-2cm} \stackrel{(a)}{=}\frac{B}{n} + \frac{1}{n}\sum_{j=i+1}^n \int_{\Scnt{j-i}{}} \E[\ell (y_j, \fal{i}{}(x_j)) | \Scnt{j}{}] - \E[\ell(y_j, \fal{i-1}{}(x_j))| \Scnt{j-1}{}]d\P(\Scnt{j-i}{}) \nonumber \\
	&\stackrel{(b)}{\leq} \frac{B}{n} + \frac{1}{n}\sum_{j=i+1}^{n}  \int_{\Scnt{j-i}{}} a_j d\P(\Scnt{j-i}{}) = \frac{B}{n} + \frac{1}{n}\sum_{j=i+1}^{n} a_j  < \frac{B + K}{n} \nonumber 
\end{align}
where $K := \sum_{i=1}^{\infty} < \infty$. In $(a)$, we write the conditional expectation as an integration of new conditional expectation in which new conditions are given for the next $j-i$ samples. While adding these new conditions, we utilize Assumption \ref{assump shuffle}. In $(b)$, we utilize Assumption \ref{assump datasets}.  
Note that $|\Lc_t(\bal) - \Lch_t(\bal)| = | X_{t,0} - X_{t,n}|$ and for every $t \in [T]$, we have $|X_{t,i} - X_{t,i-1}| < \frac{B + K}{n}$. As a result of applying Azuma-Hoeffding's inequality, we obtain 
\begin{align}
	\P(|\Lc_t(\bal)-\Lch_t(\bal)|\geq t)\leq2 e^{-\frac{nt^2}{2(B+K)^2}} \quad \forall t_1 \in [T].\nonumber
\end{align}
Let's consider $Y_t := \Lc_t(\bal)-\Lch_t(\bal)$ for $t \in [T]$. Then, $(Y_t)_{t=1}^T$ is an i.i.d. zero mean sub-gaussian random variable sequence. There exists an absolute constant $c_1 > 0$ such that $\tsub{Y_t} < \frac{c_1 (B+K)^2}{n} $ by Proposition 2.5.2 in \red{cite Roman Vers}. Applying Hoeffding's inequality, we derive
\begin{align}
	\P\left(\bigg|\frac{1}{T} \sum_{t_1=1}^T Y_{t_1} \bigg|\geq t \right) < 2e^{-\frac{cnTt^2}{(B+K)^2}} \Longrightarrow\P(|\Lch(\bal)-\Lc(\bal)|\geq t)\leq2 e^{-\frac{cnTt^2}{(B+K)^2}}
\end{align}
where $c>0$ is an absolute constant. Applying union bound over $\bAc$ and setting $t=(B+K)\sqrt{\frac{\log D+\tau}{cnT}}$, we have that for any $\bal\in\bAc$, with probability at least $1-2e^{-\tau}$,
\[
	|\Lch(\bal)-\Lc(\bal)|\leq (B+K)\sqrt{\frac{\log D+\tau}{cnT}}.
\]
\end{comment}
	Let's look at the difference: (for the sake of simplicity in the notation, we omit the subscript $t$)
\begin{align}
	|X_{t,i} - X_{t,i-1}| &= \E\bigg[\frac{1}{n}\sum_{i=1}^n \ell(y_{i},\fal{i-1}{}(\x_{i})) \bigg| \Scnt{i}{}\bigg] - \E\bigg[\frac{1}{n}\sum_{i=1}^n \ell(y_{i},\fal{i-1}{}(\x_{i})) \bigg| \Scnt{i-1}{}\bigg]\nonumber \\
	&= \frac{1}{n}\sum_{j=i}^n \E[\ell (y_j, \fal{i}{}(x_j)) | \Scnt{i}{}] - \E[\ell(y_j, \fal{i-1}{}(x_j))| \Scnt{i-1}{}] \nonumber \\
	&\leq \frac{B}{n} + \frac{1}{n}\sum_{j=i+1}^n \E[\ell (y_j, \fal{i}{}(x_j)) | \Scnt{i}{}] - \E[\ell(y_j, \fal{i-1}{}(x_j))| \Scnt{i-1}{}] \nonumber \\
	& \hspace{-2cm} \stackrel{(a)}{=}\frac{B}{n} + \frac{1}{n}\sum_{j=i+1}^n \int_{\Scnt{j-i}{}} \E[\ell (y_j, \fal{i}{}(x_j)) | \Scnt{j}{}] - \E[\ell(y_j, \fal{i-1}{}(x_j))| \Scnt{j-1}{}]d\P(\Scnt{j-i}{}) \nonumber \\
	&\stackrel{(b)}{\leq} \frac{B}{n} + \frac{1}{n}\sum_{j=i+1}^{n}  \int_{\Scnt{j-i}{}} \frac{K}{j} d\P(\Scnt{j-i}{}) = \frac{B}{n} + \frac{1}{n}\sum_{j=i+1}^{n} \frac{K}{j}  < \frac{B + K \log n}{n} \nonumber 
\end{align}
where $K := \sum_{i=1}^{\infty} < \infty$. In $(a)$, we write the conditional expectation as an integration of new conditional expectation in which new conditions are given for the next $j-i$ samples. In $(b)$, we utilize Assumption \ref{assump robust}.  
Note that $|\Lc_t(\bal) - \Lch_t(\bal)| = | X_{t,0} - X_{t,n}|$ and for every $t \in [T]$, we have $|X_{t,i} - X_{t,i-1}| < \frac{B + K}{n}$. As a result of applying Azuma-Hoeffding's inequality, we obtain 
\begin{align}
	\P(|\Lc_t(\bal)-\Lch_t(\bal)|\geq t)\leq2 e^{-\frac{nt^2}{2(B+K)^2}} \quad \forall t_1 \in [T].\nonumber
\end{align}
Let's consider $Y_t := \Lc_t(\bal)-\Lch_t(\bal)$ for $t \in [T]$. Then, $(Y_t)_{t=1}^T$ is an i.i.d. zero mean sub-gaussian random variable sequence. There exists an absolute constant $c_1 > 0$ such that $\tsub{Y_t} < \frac{c_1 (B+K \log n)^2}{n} $ by \cite[Proposition 2.5.2]{vershynin2018high}. Applying Hoeffding's inequality, we derive
\begin{align}
	\P\left(\bigg|\frac{1}{T} \sum_{t_1=1}^T Y_{t_1} \bigg|\geq t \right) < 2e^{-\frac{cnTt^2}{(B+K \log n)^2}} \Longrightarrow\P(|\Lch(\bal)-\Lc(\bal)|\geq t)\leq2 e^{-\frac{cnTt^2}{(B+K \log n)^2}}
\end{align}
where $c>0$ is an absolute constant. Applying union bound over $\bAc$ and setting $t=(B+K \log n)\sqrt{\frac{\log D+\tau}{cnT}}$, we have that for any $\bal\in\bAc$, with probability at least $1-2e^{-\tau}$,
\[
	|\Lch(\bal)-\Lc(\bal)|\leq (B+K \log n)\sqrt{\frac{\log D+\tau}{cnT}}.
\]

\red{STILL WORKING ON STEP 2 ...}

\textbf{Step 2: Consider the perturbation introduced by discretization.} Here, we relate the discrete set $\bAc$ to the continuous set $\Ac$. Following Definition~\ref{def cover}\&\ref{def distance}, let $\Ac_\eps^\Sca$ be $\eps$-cover of $\Ac$ based on distance metric $\rho_\Sca(\cdot,\cdot)$ and $\Nc(\Ac,\rho_\Sca;\eps)$ is the covering number.
Recall that $\ell(\cdot,\cdot)$ is $L$-Lipschitzness.
% , and for any $\bal\in\Ac$ and valid $\Scnt{i-1}{t}$, $\fal{i-1}{t}$ is $\Gamma$-Lipschitzness. 
For any $\bal\in\Ac$, let $\bal'\in\Ac_\eps^\Sca$ be its neighbor. Then we find
\begin{align*}
	\left|\Lch(\bal)-\Lch(\bal')\right|&=\left|\frac{1}{nT}\sum_{t=1}^T\sum_{i=1}^n\left(\ell(y_{ti},\fal{i-1}{t}(\x_{ti}))-\ell(y_{ti},\falp{i-1}{t}(\x_{ti}))\right)\right|\\
	&\leq \frac{L}{nT}\sum_{t=1}^T\sum_{i=1}^n\left|\fal{i-1}{t}(\x_{ti})-\falp{i-1}{t}(\x_{ti})\right|\\
	&=\frac{L}{\sqrt{nT}}\sqrt{\frac{1}{nT}\left(\sum_{t=1}^T\sum_{i=1}^n\left|\fal{i-1}{t}(\x_{ti})-\falp{i-1}{t}(\x_{ti})\right|\right)^2}\\
	&\leq\frac{L}{\sqrt{nT}}\sqrt{\frac{1}{nT}\sum_{t=1}^T\sum_{i=1}^n\left(\fal{i-1}{t}(\x_{ti})-\falp{i-1}{t}(\x_{ti})\right)^2}\\
	&\leq\frac{L\eps}{\sqrt{nT}}.
\end{align*}

%To continue, we introduce the \emph{worst-case} covering number. Let $\widetilde{\Sca}=\arg\sup_{\Sca}\Nc(\Ac,\rho_{\Sca};\eps)$. Then the worst-case covering number with respect to $\eps$-covers is $\Nc(\Ac,\rho_{\widetilde\Sca};\eps)$. It shows that for any achievable dataset, its $\eps$-cover has cardinality bounded by $\Nc(\Ac,\rho_{\widetilde\Sca};\eps)$. 
%Now define $\Sca'=\arg\max_{\Sca}|\Lch(\bal)-\Lch(\bal')|$, and then let $\Ac_\eps^{\Sca'}$ be its $\eps$-cover. Now consider the set 
\begin{align*}
	\left|\Lc(\bal)-\Lc(\bal')\right|&=\left|\frac{1}{nT}\sum_{t=1}^T\E_{\Sca}\left[\sum_{i=1}^n\ell(y_{ti},\fal{i-1}{t}(\x_{ti}))-\ell(y_{ti},\falp{i-1}{t}(\x_{ti}))\right]\right|\\
	&\leq
%	&\leq\sup_{\Sca}\left|\frac{1}{nT}\sum_{t=1}^T\sum_{i=1}^n\ell(y_{ti},\fal{i-1}{t}(\x_{ti}))-\ell(y_{ti},\falp{i-1}{t}(\x_{ti}))\right|\\
%	&\leq \sup_{\Sca}\frac{L}{nT}\sum_{t=1}^T\sum_{i=1}^n\left|\fal{i-1}{t}(\x_{ti})-\falp{i-1}{t}(\x_{ti})\right|
\end{align*}
\red{HOW TO BOUND $|\Lc(\bal)-\Lc(\bal')|$?}

Next, we will bound covering number in terms of worst-case Gaussian complexity $\Gct_{nT}(\Ac)$ (defined in Definition~\ref{def rad}). Inspired by \cite{tripuraneni2020theory} and letting $\widetilde{\Sca}=\arg\max_{\Sca}\Nc(\Ac,\rho_{\Sca};\eps)$, we have 
\begin{align}
	\sqrt{\log\Nc(\Ac,\rho_\Sca;\eps)}\leq\sqrt{\log\Nc(\Ac,\rho_{\widetilde\Sca};\eps)}\leq\frac{2}{\eps}\sqrt{nT}\Gch_{\widetilde\Sca}(\Ac)\leq\frac{2}{\eps}\sqrt{nT}\Gct_{nT}(\Ac).\label{cover2rad}
\end{align}
Hence, we have that with probability at least $1-2e^{-\tau}$,
\[
	|\Lch(\bal)-\Lc(\bal)|\leq|\sup_{\Sca}\Lch_\Sca(\bal)-\Lc(\bal)|\leq\frac{4B}{\eps}\Gct_{nT}(\Ac)+2B\sqrt{\frac{\tau}{nT}}\red{+}.
\]
Here we emphasize that the inequality holds for any training dataset $\Sca$.



%Applying union bound over all $T$ contexts and setting $t=\sqrt{\frac{2B^2(\log(T)+\tau)}{n}}$,
%\[
%    \P\left(\sup_{t\in[T]}\left|\Lch_t-\Lc_t\right|\geq t\right)\leq 2e^{-\tau}.
%\]
%
%Next, let $Y_t:=\Lch_t-\Lc_t$. Here, $\{Y_t\}_{t=1}^T$ are independent random variables with $\E[Y_t]=0$ and with probability at least $1-2e^\tau$, $|Y_t|\leq \sqrt{\frac{2B^2(\log(T)+\tau)}{n}}$. Then using Hoeffding's inequality we can obtain
%\[
%    \P\left(\left|\frac{1}{T}\sum_{t=1}^TY_t\right|\geq t'\right)\leq 2e^{-\frac{nTt'^2}{4B^2(\log(T)+\tau)}}+2e^{-\tau}\Longrightarrow\P\left(\left|\Lch-\Lc\right|\geq t'\right)\leq 2e^{-\frac{nTt'^2}{4B^2(\log(T)+\tau)}}+2e^{-\tau}.
%\] 
%Set $t'=\sqrt{\frac{4B^2\tau(\log(T)+\tau)}{nT}}$, and then $\P(|\Lch-\Lc|\geq t')\leq 4e^{-\tau}$. 
%
%Finally, since we consider algorithm $\bal\in\Ac_\eps$, where $\Ac_\eps$ is a discrete set with cardinality $\Nc(\Ac,\rho_\Sca;\eps)$. Applying union bound inequality over $\Ac_\eps$, we find that for all $\bal\in\Ac_\eps$
%\begin{align*}
%    \P\left(\left|\Lch(\bal)-\Lc(\bal)\right|\geq t'\right)\leq4\Nc(\Ac,\rho_\Sca;\eps)e^{-\tau}=4e^{-(\tau-\log\Nc(\Ac,\rho_\Sca;\eps))}.
%\end{align*}
%Refine the expression and we have that with probability at least $1-4e^{-\tau}$,
%\[
%    \left|\Lch(\bal)-\Lc(\bal)\right|\leq 2B\frac{\log(T\cdot\Nc(\Ac,\rho_\Sca;\eps))+\tau}{\sqrt{nT}}
%\]
% \begin{align*}
%     \P\left(\left|\frac{1}{T}\sum_{t=1}^TY_t\right|\leq t'\right)\geq \P\left(\left|\frac{1}{T}\sum_{t=1}^TY_t\right|\leq t',\sup_{t\in[T]}\left|\Lch_t-\Lc_t\right|\leq t\right)\geq .
% \end{align*}

----------------------------------

Next, we turn to bound $\Rapx$. Here, $\Lc^\st_\f=\min_{\f\in\Fc^T}\frac{1}{T}\sum_{t=1}^T\E[\ell(y_{ti},f_t(\x_{ti}))]$. Let $\Lch_\Fc(\f):=\frac{1}{nT}\sum_{t=1}^T\sum_{i=1}^n\ell(y_{ti},f_t(\x_{ti}))$ and $\hat\f:=\arg\min_{\f\in\Fc^T}\Lch_\Fc(\f)$. Following Assumption~\ref{assump erm} and applying Lemma~\ref{lemma F risk bound}, \red{with probability at least $1-2\delta$}, $\Rapx$ can be easily bounded as follows. 
\begin{align*}
	\Rapx&=\min_{\bal\in\Ac}\E[\Lch_\Sca(\bal)] - \Lc_\f^\st\\
	&=\min_{\bal\in\Ac}\E[\Lch_\Sca(\bal)] - \Lc_\Fc(\hat\f)+\Lc_\Fc(\hat\f)-\Lc_\f^\st\\
	&\leq\ept+\red{12L\Gct(\Fc)+6\sqrt{\log\frac{4T}{\delta}}\left(\frac{1+\frac{1}{\sqrt{2}}+\dots+\frac{1}{\sqrt{n}}}{n}\right)}\\
	&\leq\ept+\red{12L\Gct(\Fc)+12\sqrt{\frac{\log\frac{4T}{\delta}}{n}}}.
\end{align*}

\end{proof}


==> app/mtl_proof_v2.tex <==
\section{Proof of Theorem~\ref{thm mtl}}
\begin{definition}[Covering number ]\label{def cover} Let $\Ac:\Zc\rightarrow\R$ be a set of algorithm hypotheses. Given $\bal,\bal'\in\Ac$, and a distance metric $d(\bal,\bal')\geq0$, $\Ac_\eps=\{\bal_1,\dots,\bal_N\}$ is the $\eps$-cover of $\Ac$ with respect to the distance metric $d$ if for any $\bal\in\Ac$, there exists $\bal_i\in\Ac_\eps$ such that $d(\bal,\bal_i)\leq\eps$. Define the cardinality of the minimal $\eps$-covers as $\eps$-covering number defined by $\Nc(\Ac,d;\eps)$.  
\end{definition}
\begin{assumption}\label{assump subgaussian}
	Let $\Ac:\Zc\rightarrow\R$ be a set of algorithm hypotheses and $\Sca:=\{\Sc_t\}_{t}^T\distas\Dca$ where $\Sc_t=\{(\x_{ti},y_{ti})\}_{i=1}^n$. For any $\bal\in\Ac$, let $\yal{\Sca}=((\fal{i-1}{t}(\x_{ti}))_{i=1}^n)_{t=1}^T$. Then we assume that
	\[
		\sigma_\Ac^2:=\inf\left\{\sigma^2:\frac{1}{nT}\|\yal{\Sca}-\yalp{\Sca}\| \text{ is $\sigma^2$-subgaussian for all $\bal,\bal'\in\Ac$}\right\}<\infty.
	\]
	Then we can say $\Ac$ is $\sigma_\Ac^2$-subgaussian.
\end{assumption}
\begin{definition}[Distance metric]\label{def distance} Let $\Ac:\Zc\rightarrow\R$ be a set of algorithm hypotheses. Assume there are $T$ tasks $\Sca:=\{\Sc_t\}_{t}^T\distas\Dca$ where $\Sc_t=\{(\x_{ti},y_{ti})\}_{i=1}^n$. Following \eqref{mtl opt}, given any $\bal\in\Ac$, let $\yal{\Sca}=((\fal{i-1}{t}(\x_{ti}))_{i=1}^n)_{t=1}^T$. Then we define the distance metric of $\Ac$ by $\rho(\bal,\bal'):=\sup_{\Sca}\|\yal{\Sca}-\yalp{\Sca}\|$.
% \[
% 	\rho_\Sca(\bal,\bal'):=\inf\{\sigma:\frac{1}{nT}\left(\|\yal{\Sca}-\yalp{\Sca}\|+\|\yal{\Sc}-\yalp{\Sc}\|\right) \text{ is $\sigma^2$-subgaussian}\}.
% \]
% \[
% 	\rho_\Sca(\bal,\bal'):=\sup_\Sc\|\yal{\Sc}-\yalp{\Sc}\|~s.t.~\frac{1}{nT}\left(\|\yal{\Sca}-\yalp{\Sca}\|+\|\yal{\Sc}-\yalp{\Sc}\|\right) \text{ is $\sigma^2$-subgaussian}.
% \]
\end{definition}
\begin{theorem}[Theorem~\ref{thm mtl} restated] \label{thm mtl recap}
    Assume loss function $\ell(y,\hat y)$ takes values in $[0,B]$ and is an $L$-Lipschitz function. 
    %    Any $\fal{i-1}{t}$ generated by $\bal$ and $\Scnt{i-1}{t}\distas\Dc_t$ is a $\Gamma$-Lipschitz function.
    Let $\bah$ and $\bal^\st$ be the empirical and population solutions of \eqref{mtl opt}. Then with probability at least $1-2e^{-\tau}$, then the generalization error obeys
    \[
        \Lc_\Dca(\bah)-\Lc_\Dca(\bal^\st)\leq
    \]
\end{theorem}
\begin{proof}
Let $[n]:=\{1,2,\dots,n\}$. Recap the MTL problem which assumes that there are $T$ contexts each with $n$ in-context training samples denoted by $(\Sc_t)_{t=1}^T\distas(\Dc_t)_{t=1}^T$ where $\Sc_t=\{(x_{ti},y_{ti})\}_{i=1}^n$ and $\Sca=\bigcup_{t=1}^T\Sc_t$. As stated in Section~\ref{sec setup}, a transformer model can be seen as an algorithm $\bal$. Let $\Ac$ denote the corresponding algorithm set and then for any $\bal\in\Ac$, define training risk $\Lch_\Sca(\bal)=\frac{1}{nT}\sum_{t=1}^{T}\sum_{i=1}^n\ell(y_{ti},\fal{i-1}{t}(\x_{ti}))$ and test risk $\Lc_\Dca(\bal)=\E[\Lch_\Sca(\bal)]$. Let empirical solution $\bah=\arg\min_{\bal\in\Ac}\Lch_\Sca(\bal)$ and optimal feasible solution $\bal^\st=\arg\min_{\bal\in\Ac}\Lc_\Dca(\bal)$. For cleaner notations, in the following we drop the subscripts $\Dca$ and $\Sca$. Let $\Rgen(\bah)$ be the generalization error, where we have
\begin{align}
	\Rgen(\bah)&=\Lc(\bah)-\Lc(\bal^\st)\\
	&=\underset{a}{\underbrace{\Lc(\bah)-\Lch(\bah)}}+\underset{b}{\underbrace{\Lch(\bah)-\Lch(\bal^\st)}}+\underset{c}{\underbrace{\Lch(\bal^\st)-\Lc(\bal^\st)}}.
\end{align}
Since $\bah$ is the minimizer of empirical risk, intuitively we have $b\leq0$. In the following, we consider the concentration problem that for any $\bal\in\Ac$, how to upper bound $|\Lc(\bal)-\Lch(\bal)|$. 

% \textbf{Step 1: We start with the concentration bounds for any algorithm $\bal$.} 
Firstly we consider the problem that given any $\bal\in\Ac$, how $|\Lc(\bal)-\Lch(\bal)|$ can be bounded.
% Following Definition~\ref{def cover}\&\ref{def distance}, let $\Ac_\eps$ be $\eps$-cover of $\Ac$ based on distance metric $\rho_\Sca(\cdot,\cdot)$ and $\Nc(\Ac,\rho_\Sca;\eps)$ is the covering number. 
%Define $\Lch_t(\bal)=\sum_{i=1}^n\ell(y_{ti},\fal{i-1}{t}(\x_{ti}))$ and $\Lc_t(\bal)=\E[\Lch_t(\bal)]$. Then we have that $\Lch=\frac{1}{T}\sum_{t=1}^T{\Lch_t}$ and $\Lc=\frac{1}{T}\sum_{t=1}^T\Lc_t$. 
Let us define the loss for each task separately as follows.
\begin{align}
	&\Lch_t(\bal) :=\frac{1}{n}\sum_{i=1}^n \ell(y_{ti},\fal{i-1}{t}(\x_{ti})), \quad \text{and} \nonumber \\
	&\Lc_t(\bal) :=\E_{\Sc_t}\left[\Lch_t(\bal)\right]= \E_{\Sc_t}\left[\frac{1}{n}\sum_{i=1}^n\ell(y_{ti},\fal{i-1}{t}(\x_{ti}))\right], \quad \forall t \in [T]. \nonumber
\end{align}
Define the random variables $X_{t,i}=\E[\Lch_t(\bal)|\Scnt{i}{t}]$ for $i \in [n]$ and $t \in [T]$, that is, $X_{t,i}$ is the expectation over $\Lch_t(\bal)$ given training data of $\Scnt{i}{t}=\{(\x_{tj},y_{tj})\}_{j=1}^i$. Then we have that $X_{t,n} = \E[\Lch_t(\bal)|\Scnt{n}{t}]=\Lch_t(\bal)$. Let $X_{t,0} = \E[\Lch_t(\bal)]$. Then, for every $t$ in $[T]$, the sequences $\{X_{t,0}, X_{t,1}, 
\dots, X_{t,n}\}$ are Martingale sequences with respect to $\E[X_{t,i} | \Scnt{i-1}{t}]= X_{t,i-1}$. 

For the sake of simplicity in the notation, we omit the subscript $t$ for $\x,y$ and $\Sc$ in the following. Then we have
\begin{align*}
	X_{t,i}&=\E\bigg[\frac{1}{n}\sum_{j=1}^n \ell(y_{j},\fal{j-1}{}(\x_{j})) \bigg| \Scnt{i}{}\bigg]\\
	&=\frac{1}{n}\sum_{j=1}^{i}\ell(y_{j},\fal{j-1}{}(\x_{j}))+\frac{1}{n}\sum_{j=i+1}^{n}\E\left[\ell(y_{j},\fal{j-1}{}(\x_{j}))\bigg|\Scnt{i}{}\right]
\end{align*}
Next, we look at the difference of neighbors. 
\begin{align}
	&|X_{t,i} - X_{t,i-1}| = \left|\E\bigg[\frac{1}{n}\sum_{j=1}^n \ell(y_{j},\fal{j-1}{}(\x_{j})) \bigg| \Scnt{i}{}\bigg] - \E\bigg[\frac{1}{n}\sum_{j=1}^n \ell(y_{j},\fal{j-1}{}(\x_{j})) \bigg| \Scnt{i-1}{}\bigg]\right|\nonumber \\
	% &\leq\scalemath{0.8}{\frac{1}{n}\left|\ell(y_{i},\fal{i-1}{}(\x_{i}))-\E\left[\ell(y_{i},\fal{i-1}{}(\x_{i}))\bigg|\Scnt{i-1}{}\right]\right|+\frac{1}{n}\sum_{j=i+1}^n\left| \E\left[\ell (y_j, \fal{j-1}{}(\x_j)) \bigg| \Scnt{i}{}\right] - \E\left[\ell(y_j, \fal{j-1}{}(\x_j))\bigg| \Scnt{i-1}{}\right]\right|} \nonumber \\
	&\leq\scalemath{0.8}{\frac{1}{n}\sum_{j=i}^n\left| \E\left[\ell (y_j, \fal{j-1}{}(\x_j)) \bigg| \Scnt{i}{}\right] - \E\left[\ell(y_j, \fal{j-1}{}(\x_j))\bigg| \Scnt{i-1}{}\right]\right|} \nonumber \\
	&\stackrel{(a)}{\leq}\scalemath{0.8}{\frac{B}{n} + \frac{1}{n}\sum_{j=i+1}^n \left|\E\left[\ell (y_j, \fal{j-1}{}(\x_j)) \bigg| \Scnt{i}{}\right] - \E\left[\ell(y_j, \fal{j-1}{}(\x_j))\bigg| \Scnt{i-1}{}\right]\right|} \nonumber \\
	& \stackrel{(b)}{\leq}\scalemath{0.8}{\frac{B}{n} + \frac{1}{n}\sum_{j=i+1}^n \int \left|\E\left[\ell (y_j, \fal{j-1}{}(\x_j)) \bigg| \Scnt{i}{}+\Scnt{i+1:j-1}{\Delta}\right] - \E\left[\ell(y_j, \fal{j-1}{}(\x_j))\bigg| \Scnt{i-1}{}+\Scnt{i:j-1}{\Delta}\right]\right|d\P(\Scnt{i:j-1}{\Delta})} \nonumber \\
	&\stackrel{(c)}{\leq}\scalemath{0.8}{ \frac{B}{n} + \frac{1}{n}\sum_{j=i+1}^{n}  \int \frac{K}{j-1} d\P(\Scnt{i:j-1}{\Delta}) = \frac{B}{n} + \frac{1}{n}\sum_{j=i+1}^{n} \frac{K}{j-1}< \frac{B + K \log n}{n}}. \nonumber 
\end{align}
for $i<n$. Here, $(a)$ is from the fact that loss function $\ell(\cdot,\cdot)$ is bounded by $B$. In $(b)$, we write the conditional expectation as an integration of new conditional expectation in which new conditions are given for the next samples indexed from $i$ to $j-1$ shown as $\Scnt{i:j-1}{}$($\Sc_{i:j-1}=\emptyset$ if $i>j-1$). In $(c)$, we utilize Assumption \ref{assump robust}. Intuitively we have 
\[
|X_{t,n} - X_{t,n-1}|=\frac{1}{n}\left|\ell(y_{n},\fal{n-1}{}(\x_{n}))-\E\left[\ell(y_{n},\fal{n-1}{}(\x_{n}))\bigg|\Scnt{n-1}{}\right]\right|\leq\frac{B}{n}< \frac{B + K \log n}{n}.
\]
Note that $|\Lc_t(\bal) - \Lch_t(\bal)| = | X_{t,0} - X_{t,n}|$ and for every $t \in [T]$, we have $\sum_{i=1}^{n}|X_{t,i} - X_{t,i-1}|^2\leq\frac{(B+K\log n)^2}{n}$. As a result of applying Azuma-Hoeffding's inequality, we obtain 
\begin{align}
	\P(|\Lc_t(\bal)-\Lch_t(\bal)|\geq \tau)\leq2 e^{-\frac{n\tau^2}{2(B+K\log n)^2}}, \quad \forall t \in [T].\nonumber
\end{align}
Let's consider $Y_t := \Lc_t(\bal)-\Lch_t(\bal)$ for $t \in [T]$. Then, $(Y_t)_{t=1}^T$ is an i.i.d. zero mean sub-Gaussian random variable sequence. There exists an absolute constant $c_1 > 0$ such that $\tsub{Y_t} < \frac{c_1 (B+K\log n)^2}{n} $ by \cite[~Proposition 2.5.2]{vershynin2018high} Applying Hoeffding's inequality, we derive
\begin{align}
	\P\left(\bigg|\frac{1}{T} \sum_{t=1}^T Y_{t} \bigg|\geq \tau \right) < 2e^{-\frac{cnT\tau^2}{(B+K\log n)^2}} \Longrightarrow\P(|\Lch(\bal)-\Lc(\bal)|\geq \tau)\leq2 e^{-\frac{cnT\tau^2}{(B+K\log n)^2}}
\end{align}
where $c>0$ is an absolute constant. Therefore, we have that for any $\bal\in\Ac$, with probability at least $1-2\delta$,
\[
	|\Lch(\bal)-\Lc(\bal)|\leq (B+K\log n)\sqrt{\frac{\log(1/\delta)}{cnT}}.
\]

Next, we turn to bound $\sup_{\bal\in\Ac}|\Lc(\bal)-\Lch(\bal)|$, where $\Ac$ is a continuous search space. Then it can be simply bounded by
\begin{align*}
	\sup_{\bal\in\Ac}|\Lc(\bal)-\Lch(\bal)|=\sup_{\bal\in\Ac}\left|\E_\Sc[\Lch_\Sc(\bal)]-\Lch(\bal)\right|\leq\E_\Sc\left[\sup_{\bal\in\Ac}\left|\Lch_\Sc(\bal)-\Lch(\bal)\right|\right].
\end{align*}
Let $g(\bal):=\Lch_\Sc(\bal)-\Lch(\bal)$ and now we are focusing on bounding $\E[\sup_{\bal\in\Ac}|g(\bal)|]$. Following Definition~\ref{def distance}, let $D:=\sup_{\bal,\bal'\in\Ac}\rho(\bal,\bal')$. For $\eps>0$, let $\Ac_\eps$ be $\eps$-cover of $\Ac$ in terms of distance metric $\rho$. Therefore, $\Ac_\eps$ is a discrete set with cardinality $|\Ac_\eps|:=\Nc(\Ac,\rho,\eps)$. Let $K:=\min\{k:2^k\geq D\}$. Denote $\Uc_0:=\Ac_\eps$, and for any $k\in[K]$, let $\Uc_k$ denote the minimal $2^k\eps$ cover of $\Uc_{k-1}$. Since $\Uc_K\subseteq\Uc_{K-1}\cdots\subseteq\Uc_0 \subset \Ac$, we have $|\Uc_k| = \Nc(\Uc_{k-1},\rho,2^{k}\eps) \leq \Nc(\Ac, \rho, 2^k\eps)$ and $|\Uc_K|\leq\Nc(\Ac, \rho, D)=1$. Now, let $\bal^k\in\Uc_k$ be any sample from $\Uc_k$, then we have
\[
	\left|g(\bal^0)-g(\bal^K)\right|\leq\left|g(\bal^0)-g(\bal^1)\right|+\cdots+\left|g(\bal^{K-1})-g(\bal^K)\right|,
\]
and therefore,
\begin{align*}
	\E\left[\max_{\bal^0\in\Uc_0}\left|g(\bal^0)-g(\bal^K)\right|\right]
	% &\leq\max_{\bal^0\in\Uc_0,\bal^1\in\Uc_1}\left|g(\bal^0)-g(\bal^1)\right|+\cdots+\max_{\bal^{K-1}\in\Uc_{K-1}}\left|g(\bal^{K-1})-g(\bal^K)\right|\\
	&\leq\sum_{k=0}^{K-1}\E\left[\max_{\bal^{k}\in\Uc_{k},\bal^{k+1}\in\Uc_{k+1}}\left|g(\bal^{k})-g(\bal^{k+1})\right|\right]\\
	&\leq\sum_{k=0}^{K-1}\E\left[\max_{\bal,\bal'\in\Uc_{k}}\left|g(\bal)-g(\bal')\right|\right].
\end{align*}
To continue, we first prove that $g(\bal)-g(\bal')$ for any $\bal,\bal'\in\Uc_k$ is subgaussian. Let $\Sc:=\{\Sc_t\}_{t=1}^T\distas\Dca$ be any set, then we have
\begin{align*}
	\left|\Lch_\Sc(\bal)-\Lch_\Sc(\bal')\right|&=\left|\frac{1}{nT}\sum_{t=1}^T\sum_{i=1}^n\left(\ell(y_{ti},\fal{i-1}{t}(\x_{ti}))-\ell(y_{ti},\falp{i-1}{t}(\x_{ti}))\right)\right|\\
	&\leq \frac{L}{nT}\sum_{t=1}^T\sum_{i=1}^n\left|\fal{i-1}{t}(\x_{ti})-\falp{i-1}{t}(\x_{ti})\right|\\
	&\leq\frac{L}{\sqrt{nT}}\sqrt{\sum_{t=1}^T\sum_{i=1}^n\left(\fal{i-1}{t}(\x_{ti})-\falp{i-1}{t}(\x_{ti})\right)^2}\\
	&\leq\frac{L\eps}{\sqrt{nT}}.
\end{align*}
\begin{align*}
	g(\bal)-g(\bal')&=\Lch_\Sc(\bal)-\Lch_\Sc(\bal')+\Lch(\bal)-\Lch(\bal')\\
	&\leq
\end{align*}



------------------------------------

Let $g(\bal):=\Lch_\Sc(\bal)-\Lch(\bal)$ and now we are focusing on bounding $\E[\sup_{\bal\in\Ac}|g(\bal)|]$. Following Definition~\ref{def distance}, let $D:=\sup_{\bal,\bal'\in\Ac}\rho(\bal,\bal')$. For $\eps>0$, let $\Ac_\eps := \{ \bal_1, \bal_2, \dots, \bal_N\}$ be $\eps$-cover of $\Ac$ in terms of distance metric $\rho$. Therefore, $\Ac_\eps$ is a discrete set with cardinality $|\Ac_\eps|:=\Nc(\Ac,\rho,\eps) = N$.  For any $\bal \in \Ac$, we can find some $\bal_i$ such that $\rho(\bal, \bal_i) < \eps$ where $\bal_i \in \Ac_\eps$.
\begin{align}
	g(\bal) - g(\bal_1) &= (g(\bal) - g(\bal_i)) + (g(\bal_i) - g(\bal_1)) \nonumber \\
	& \leq \sup_{\bal, \bal^{'} : \rho(\bal, \bal^{'}) < \eps} (g(\bal) - g(\bal^{'})) + \max_{i = 1,2,\dots,N} |g(\bal_i) - g(\bal_1)| \nonumber
\end{align}
If we do the same thing $\tilde{\bal} \in \Ac$, then we obtain the following:
\begin{align}
	\sup_{\bal, \tilde{\bal} \in \Ac} &(g(\bal) - g(\tilde{\bal}) ) \nonumber \\
	&\leq 2 \sup_{\bal, \bal^{'} : \rho(\bal, \bal^{'}) < \eps} (g(\bal) - g(\bal^{'})) + 2 \max_{i = 1,2,\dots,N} |g(\bal_i) - g(\bal_1)| \nonumber
\end{align} 
Now, let $\Ac_k$ denote the $2^{-k}\eps$-cover of $\Ac_\eps$. Since $\Ac_\eps\subset\Ac$, we have $|\Ac_k|=\Nc(\Ac_\eps,\rho,2^{-k}\eps)\leq\Nc(\Ac,\rho,2^{-k}\eps)$. Since $\Ac_\eps$ is finite, there exists $L \in \mathbb{R}$ such that $\Ac_\eps = \Ac_L$. Inspired by \red{the book}, let us define the following map for every $m = 1,2, \dots, L$:
\begin{align}
	\pi_m(\bal) = \arg \min_{\bal^{'} \in \Ac_m} \rho(\bal, \bal^{'})
\end{align} 
As a result, for any $\bal \in \Ac_\eps$, we can generate a sequence $\{ \gamma^1, \gamma^2, \dots, \gamma^L\}$ such that $\gamma^L := \bal$ and $\gamma^{m-1} := \pi_{m-1}(\gamma^m)$ for $m = L, L-1, \dots, 2$. Then, we derive the following:
\begin{align}
	g(\bal) - g(\gamma^1) = \sum_{m=2}^L g(\gamma^m) - g(\gamma^{m-1})
\end{align}
For any $\tilde{\bal} \in \Ac_\eps$, we can generate a similar sequence $\{\tilde{\gamma}^1, \tilde{\gamma}^2, \dots, \tilde{\gamma}^L\}$. Then we obtain the following:
\begin{align}
	|g(\bal) - g(\tilde{\bal})| \leq |g(\gamma^1) - g(\tilde{\gamma}^1) s
\end{align}






Therefore, we have 


\end{proof}


==> sec/comments.tex <==
\subsection*{Dimitris' feedback: Main takeaway. Concrete stability bounds for TF}
\begin{myenumerate}
\item the $\rho(alg, alg)$ treats $f_S(alg)$ as an n dimensional vector, where the ith coordinate is the prediction given that the algorithm has observed up to sample i-1? so it's some kind of autoregressive “prediction” distance between two algorithms?
\item \textbf{robustness vs stability phrasing:} why do you call asm 3 robustness, isnt this stability in eq(1)?
\item \textbf{theorem too complex (already simplified a bit):} how do you get (2) from (1)? (I would suggest having an informal version of Thm4, if we'll send that to ICML)
\item in the experiments are you actually running on a TF? the setting is not really clarified.\\\textbf{we should give more details on this}
\item we can short of hack some TF into Asm3 since again the algorithm, whatevwr it does, is encoded in teh weigths of a TF
\begin{itemize} 
\item it may depend exponentially on the depth, but ppl don't use really deep TFs in practice
\item \textbf{Agreed, it is the input-lipschitzness of the TF basically.} 
\end{itemize}
%\item if you also assume that the TF is using mask attention, then if the replaced sample z_j is at position j, then the difference of the outputs till then it will be 0
\item If your first layer is an attention layer, then that $z_j$ you resampled (not sure if you resample it or if it's worst case), it appears on the $j_th$ column \& row of attention matrix $X^\top Q^\top KX$. The jth row will be $[z_jQKz_1~z_jQKz_2~…~z_jQKz_n]$ and the jth column $[z_1QKz_j~z_2QKz_j~…~z_nQKz_j]'$. The remaining n choose 2 elements are the same as before. So if we assume something about the distribution of $z_j$ (eg it's not worst case), then it should be easy to show that it doesnt affect significantly the “distribution” that the softmax spits out, apart from 1 column, the jth which is all messed up. All other columnbs, only have 1 element off (distributional assumptions shoudl take care of how “much” the softmax output on all other columns changes). What this means tho is perhaps really bad will happed downstream, because if $\Sigma$ was the attention matrix (after the softmax) before sampling $z_j$, and $\Sigma_j$ the new one, then we can think of it “mixing” columns of X (or $X_j$). So $X_j\Sigma_j$ and $X\Sigma$ should be close, e.g.~$X_j\Sigma_j \sim X\Sigma +(XE_j+(X-X_j)*\Sigma)$, where $E_j$ is the column that's different between $\Sigma_j$ and $\Sigma$. Note that if things are ``regular'' norm-wise, then i think $\|XE_j+(X-X_j)\Sigma\|\sim O(1/n)$ [dimension is hidden here], since $E_j$ is nearly zero everywhere apart form one column and $X-X_j$ is also zero everywhere apart from teh jth column. Call $(XE_j+(X-X_j)*\Sigma)$ just $E$. Since the only column “off” is the jth the prediction will differ as follows $||VRelu(W X\Sigma) - VRelu(W X\Sigma+WE)||\sim O(||V|| * ||W|| * ||E||)$
\item \textbf{Concrete stability bound for TF to make paper stronger:} an easy stability bound would look something like $d^\text{depth}/n$ or something since the dimension of V and W does not depend on n and the norm of E in proportion to X should be around O(1/n)
\item in the above you don't need distributional assumptions on $||z_j||$ apart from an upper bound on it but distributional assumptions do help to get a good lower bound on ||Z||
\item \textbf{Picking up distributional prior:} there are some cases in LLMs where you only need the x to prompt it not y’s like you give it x1 x2 x3 and predicts the correct label for $x_\text{test}$ so it’s almost as if it has learnt something similar according to $x_i$s \\(\textbf{We are in the process of improving the transfer section})

\end{myenumerate}




%\footnote{We remark that this transformer is }


















==> sec/fig_diverse.tex <==
\begin{figure}
	\centering
	% \vspace{-20pt}
	\begin{minipage}{0.31\textwidth}
		\centering
		\begin{tikzpicture}
		\centering
		\node at (0,0) {\includegraphics[scale=0.25]{figs/mtl2.pdf}};
		\node at (0, -2.2) {\small{(a) Each task with single trajectory}}; %\label{fig:noisy linear}
		\end{tikzpicture}
	\end{minipage}
	\hspace{5pt}
	\begin{minipage}{0.31\textwidth}
		\centering
		\begin{tikzpicture}
			\centering
			\node at (0,0) {\includegraphics[scale=0.25]{figs/mtl_meta_all.pdf}};
			\node at (0.1, -2.2) {\small{(b) Each task with multiple trajectories}}; %\label{fig:weighted}
		\end{tikzpicture}
	\end{minipage}
	\hspace{5pt}
	\begin{minipage}{0.31\textwidth}
		\centering
		\begin{tikzpicture}
			\centering
			\node at (0,0) {\includegraphics[scale=0.25]{figs/diverseT20_meta_unit.pdf}};
			\node at (0, -2.2) {\small{(c) Close \emph{vs} far away tasks}}; %\label{fig:dynamic}
		\end{tikzpicture}
	\end{minipage}
	\vspace{-7pt}
	\caption{\small{Experiments of MTL and transfer learning risks and task diversity simulation. We run in-context learning with fixed $T<\infty$ under different scenarios where each task is trained with  a single trajectory (a), or multiple trajectories (b), and investigate the role of task diversity in (c). Details are in Section \ref{sec exp}.}}\label{fig:diverse}
	\vspace{-10pt}
	\end{figure}
	


==> sec/fig_dynamic.tex <==
%\begin{figure}
%	\centering
%	\begin{minipage}{0.35\textwidth}
%		\centering
%		\begin{tikzpicture}
%		\centering
%		\node at (0,0) {\includegraphics[scale=0.3]{figs/dynamic_partial.pdf}};
%		\node at (0, -2.5) {\small{(a) ICL \emph{vs} least squares}}; 
%		\end{tikzpicture}
%	\end{minipage}
%	\hspace{30pt}
%	\begin{minipage}{0.35\textwidth}
%		\centering
%		\begin{tikzpicture}
%			\centering
%			\node at (0,0) {\includegraphics[scale=0.3]{figs/dynamic_partial_ridge.pdf}};
%			\node at (0.1, -2.5) {\small{(b) ICL \emph{vs} optimal ridge solutions}}; 
%		\end{tikzpicture}
%	\end{minipage}
%	\vspace{-7pt}
%	\caption{\small{Dynamical system experiments. Here, (a) is exactly the same as Fig.~\ref{fig:main_exp}(b)} and (b) compares ICL to the optimal ridge regressions. }\label{fig:dynamic}
%	\vspace{-10pt}
%	\end{figure}


\begin{figure}
	\centering
	\begin{minipage}{0.35\textwidth}
		\centering
		\begin{tikzpicture}
		\centering
		\node at (0,0) {\includegraphics[scale=0.3]{figs/dynamic_partial.pdf}};
		\node at (0, -2.5) {\small{(a) ICL \emph{vs} least squares}}; 
		\end{tikzpicture}
	\end{minipage}
	\hspace{30pt}
	\begin{minipage}{0.35\textwidth}
		\centering
		\begin{tikzpicture}
			\centering
			\node at (0,0) {\includegraphics[scale=0.3]{figs/dynamic_partial_ridge.pdf}};
			\node at (0.1, -2.5) {\small{(b) ICL \emph{vs} optimal ridge solutions}}; 
		\end{tikzpicture}
	\end{minipage}
	\vspace{-7pt}
	\caption{\small{Dynamical system experiments. Here, (a) is exactly the same as Fig.~\ref{fig:main_exp}(b)} and (b) compares ICL to the optimal ridge regressions. }\label{fig:dynamic}
	\vspace{-10pt}
	\end{figure}

==> sec/intro_Nov29.tex <==
\begin{abstract}%
Prompt-based learning is emerging as one of the fundamental features of transformers and allows for adapting the model through its input interface. In-context learning is an intriguing instance of prompting where a transformer model admits a sequence of features as its input and makes inference based on this sequence on-the-fly. This \emph{implicit training} over input features is in contrast to explicitly tuning the model weights based on the features. Inspired by recent literature, in this work, we formalize in-context learning as an \emph{algorithm learning} problem where we treat the transformer model as a meta ML algorithm that can be specialized to implement a target algorithm during the training phase. We first explore the statistical aspects of this abstraction through the lens of multitask learning: We obtain generalization bounds when the input prompt is (1) a sequence of i.i.d.~(input, label) pairs or (2) a trajectory arising from a stable dynamical system. Our bounds require non-standard arguments where the stability of transformer's algorithm controls martingale concentration. Secondly, we use our abstraction to formally motivate that transformers can act as AutoML algorithms and perform model selection across different hypothesis classes. Finally, our numerical evaluations demonstrate that transformers can indeed implement near-optimal algorithms on insightful regression problems with i.i.d.~and dynamic data.

%such as optimally-weighted ridge regression or 

% for insightful regression problems with i.i.d.~or dynamic data.
%and system identification problems.

%that transformers can implement optimally weighted ridge regression 
%our \emph{algorithm learning}
%Inspired by successful applications in RL and AutoML, i
%Recent works demonstrated 

%In this work, we 

%spired by the remarkable in-context learning ability 


% and enables transformer to serve as a prompt-conditioned . 

%Success of in-context inference is inherently tied to meta-learning where transformer is trained on a large number of autoregressive tasks.

%In essence, the model implicitly trains on the prompt as the training This is in contrast to training the model

%Essentially, it illustrates the ability of a transformer 

% features are provided through the prompt and the model makes
\end{abstract}
% as it provides a natural way to interact with large language models. 

\begin{keywords}%
in-context learning, generalization, model-selection, system identification, transformer
\end{keywords}


\red{
\begin{itemize}
  \item Limit the main text (not counting references) to 10 PMLR-formatted pages, using this template.
  \item Include {\em in the main text} enough details, including proof details, to convince the reviewers of the contribution, novelty and significance of the submissions.
\end{itemize}
}

\section{Introduction}

\paragraph{Contributions:} 
\subsection{Related work}

==> sec/setup__backup_.tex <==
\section{Problem Setup}\label{sec setup}
\noindent\textbf{Notation. } Let $[n]$ denote set $\{1,2,\dots,n\}$.

Let $\Xc$ denote the feature space and assume labels are in $\R$. Let $\Fc:\Xc\rightarrow\R$ be a set of prediction hypotheses (e.g.,~linear models, neural nets, etc.). Denote $\Dc_\Xc$ as a distribution over $\Xc$ and $\Dc_{\Fc}$ as a distribution over $\Fc$. 
% Then given any $f\in\Fc$, we can generate the context samples $(\x,y)$'s by $y=f(\x)+z$ where $\x\distas\Dc_\Xc$ and $z$'s are zero-mean random variables with bounded sub-Gaussian norm. 
Let $\ell(y,\hat{y}):\R\times \R\rightarrow[0,1]$ be a loss function.

% a $n$-length context can be generated by $\xp{n}=(\x_1,y_1,\dots \x_{n-1},y_{n-1},\x_{n})$, where $\x_i\distas\Dc_\Xc$, $y_i=f(\x_i)+z_i\in\R$ and $z_i$'s are zero-mean random variables with bounded sub-Gaussian norm.

During MTL phase, suppose we are given $T$ tasks associated with $(f_t)_{t=1}^T\distas\Dc_{\Fc}$, and each contains $n$ in-context samples. Then the training dataset of $t$'th context can be denoted by $\Sn{t}=\{(\x_{ti},y_{ti})\}_{i=1}^n\distas\Dc_t$. Here, $\Dc_t$ obeys $\x_{ti}\distas\Dc_\Xc$, $y_{ti}=f_t(\x_{ti})+z_{ti}$ and $z_{ti}\distas\Dc_z$, where $\Dc_z$ is a zero-mean distribution with bounded sub-Gaussian norm. Here, we assume i.i.d. in-context examples and same sample size $n$ for all tasks for clean exposition. 
Let $\Sca=\bigcup_{t=1}^T\Sc_t$ and $\Dca=\{\Dc_t\}_{t=1}^T$. We model in-context learning with transformers as follows. Let $\TF(\cdot)$ be a transformer that admits a prompt sequence $\xp{i}=(\x_1,y_1,\x_2,y_2,\dots \x_{i-1},y_{i-1},\x_{i})$ and outputs a prediction $\yh_i=\TF(\xp{i})$.  Let $\Xc^{(i)}$ denote the $i$ times Cartesian product of space $\Xc$. Then,  $\TF(\cdot)$ has input space $\bigcup_{i=1}^\infty\Xc^{(i)}$ since transformer can take any length of sequence as inputs, which is hard to analyze. To simplify, we abstract it out as an algorithm that maps datasets to a prediction hypothesis. Concretely, let $\Ac$ be a set of algorithm hypotheses such that algorithm $\bal\in\Ac$ maps datasets of form $\Sc^{(i)}=\{(\x_j,y_j)\}_{j=1}^{i}$ into a prediction $\fal{i}{}$. Then, we propose representing $\TF$ via
\[
\TF(\xp{i+1})=\fal{i}{}(\x_{i+1})
\]
\noindent\textbf{Remark.} Here, $\fal{i}{}:\Xc\rightarrow\R$ is a prediction function determined by algorithm $\bal$ and previously observed dataset $\Sc^{(i)}$. Therefore, given any $\bal\in\Ac$, the predictions change with prompts. 

Given training samples $\Sca$ and the loss function $\ell(\cdot,\cdot)$, the in-context learning problem can be interpreted as searching for the optimal algorithm $\bal\in\Ac$, and the objective function is formulated as follows.
\begin{align}
    \bah=\arg\min_{\bal\in\Ac}\Lch_{\Sca}(\bal):=\frac{1}{nT}\sum_{t=1}^T\sum_{i=1}^n \ell(y_{ti},\underbrace{\fal{i-1}{t}(\x_{ti})}_{:=\TF({\xpt{i}{t}})}).\label{mtl opt}
\end{align}
Here, $\Sn{t}^{(i-1)}=\{(\x_{tj},y_{tj})\}_{j=1}^{i-1}\subset\Sn{t}$ and $\xpt{i}{t}=(\x_{t,1},y_{t,1},\dots \x_{t,i-1},y_{t,i-1},\x_{ti})$. Let $\Sc^{(0)}=\emptyset$. Define the population risk over training contexts $(f_t)_{t=1}^T$ as $\Lc_\Dca(\bal)=\E[\Lch_\Sca(\bal)]$, then we are interested in deriving the excess MTL test risk
%\begin{align}
%    \Rmtl(\bah)&=\Lc_\Dca(\bah)-\Lc^\st_{\f}\\
%    &=\underset{\text{generalization error}}{\underbrace{\Lc_\Dca(\bah)-\Lc_\Dca(\bal^\st)}} + \underset{\text{}}{\underbrace{\Lc_\Dca(\bal^\st) - \Lc^\st_\Ac}}+ \underset{\text{approximation error}}{\underbrace{\Lc^\st_\Ac - \Lc^\st_{\f}}}\label{mtl risk}
%\end{align}
% \begin{align}
%     \Rmtl(\bah)&=\Lc_\Dca(\bah)-\Lc^\st_{\f}\\
%     &=\underset{\text{generalization error}}{\underbrace{\Lc_\Dca(\bah)-\Lc_\Dca(\bal^\st)}} + \underset{\text{approximation error}}{\underbrace{\Lc_\Dca(\bal^\st) - \Lc^\st_{\f}}}\label{mtl risk}
% \end{align}
% where $\bal^\st=\arg\min_{\bal\in\Ac}\Lc_\Dca(\bal)$. 
\begin{align}
    \Rmtl(\bah)=\Lc_\Dca(\bah)-\Lc^\st_\Dca\label{mtl risk}
\end{align}
where $\Lc^\st_\Dca=\min_{\bal\in\Ac}\Lc_\Dca(\bal)$. 
% and \red{generalization error arises from the fact that each context has finite sample size $n$, and it will vanish if $n\rightarrow\infty$}. 
% Let $\f:=[f_1,\dots,f_T]\in\Fc^T$ and \red{$\Lc^\st_{\f}:=\frac{1}{T}\sum_{t=1}^T\E[\ell(y_{ti},f_t(\x_{ti}))]$}, then the approximation error captures how the optimal solution $\bal^\st$ performs over the $T$ contexts compared to the ground truth minimization $\Lc^\st_{\f}$. 



% This term is related to the transformer model selection. 
% Thus, $\bal_{\Sn{ti}}(\xt{t}_i)$ corresponds to the transformer prediction with input prompt $\xp{ti}=(\xt{t}_0,\yt{t}_0,\dots \xt{t}_{i-1},\yt{t}_{i-1},\xt{t}_i)$.



% In this work, we will be working with prompt sequences obtained by i.i.d.~(feature, label) pairs. Thus, we are naturally interested in algorithms that can (approximately) minimize a regularized empirical risk over $\Sn{n}$. 

Next we consider a zero-shot transfer learning. Concretely, assume a target task $f_\Tc\in\Fc$ and dataset $\Sc=\{(\x_i,y_i)\}_{i=1}^n$ where $y_i=f_\Tc(\x_i)+z_i$, $\x_i\distas\Dc_\Xc$ and $z_i\distas\Dc_\Zc$. Given a prompt sequence $\xp{i}=(\x_1,y_1,\dots,\x_{i-1},y_{i-1},\x_{i})$, we aim to predict $\hat y_i~(i\in[n])$ directly without training. Following the MTL argument, set $\hat y_i=\falh{i-1}{\Tc}(\x_{i})$, and then the excess transfer learning test risk can be defined by
\red{
\begin{align}
    R_\Tc(\bah)&=\Lc_\Tc(\bah)-\Lc_\Tc^\st\label{tf risk}\\
    &=\underset{\text{generalization error introduced by MTL}}{\underbrace{\Lc_\Tc(\bah)-\Lc_\Tc(\bal^\st)}}+\underset{\text{related to task diversity}}{\underbrace{\Lc_\Tc(\bal^\st)-\Lc_{\Tc}(\bal^\stt)}}+\underset{\text{approximation error}}{\underbrace{\Lc_{\Tc}(\bal^\stt)-\Lc_\Tc^\st}}.
\end{align}
Here, $\bal^\stt=\arg\min_{\bal\in\Ac}\E_{\f\sim\Dc^{T}_\Fc}[\Lc_\Dca(\bal)]$ and $\Lc_\Tc^\st:=\E_{\Dc_\Tc}[\ell(y,f_\Tc(\x))]$.
}
%
%we already 
%each with $n$ samples data distribution $\{\Dc_t\}_{t=1}^T$, that is  $\{\Sn{t}\}_{t=1}^T$ where $\Sn{t}=\{(\x_i^{(t)},y_i^{(t)})\}_{i=1}^n$. Here, we assume that $y_i^{(t)}=f_t(\x_i^{(t)})$ where $(f_t)_{t=1}^T\distas \Dc_{\Fc}$ and sample associated datasets $\Sca=(\Sn{t})_{t=1}^T\sim (\Dn{t})_{t=1}^T$ as above. Also sample $f_\new\sim \Dc_\Fc$ and associated $\Sn{\new}\distas\Dn{\new}$ in the same way. Here, $\Sn{\new}$ will be our test dataset. 

% \noindent\textbf{In-Context data:} Let $\Dn{t}$ be the (feature, label) distribution associated with the $t$'th context. $\Sn{t}=(\xt{t}_i,\yt{t}_i)_{i=1}^n\in\Xc\times \R$ be the $t$'th dataset sampled i.i.d.~from $\Dn{t}$. 

% \footnote{We initially formulate the problem with context being sampled randomly from $\Dc_{\Fc}$. Later on, this can be extended to deterministic set of contexts through notions such as task-diversity.}\smallskip

% \smallskip

% \noindent\textbf{Transformers as algorithms:} We model in-context learning with transformers as follows. Let $\TF(\cdot)$ be a transformer that admits a prompt sequence $\xp{n}=(\x_1,y_1,\x_2,y_2,\dots \x_{n-1},y_{n-1},\x_{n})$ and outputs a prediction $\yh_n=\TF(\xp{n})$. 




% \smallskip



% We will develop our main results for a realizable setting where each context is linked to a hypothesis within $\Fc$.

%\begin{definition} We say $\Dn{t}$ is \textbf{realizable} if $(y_t,\x_t)\sim \Dn{t}$ obeys $\x_t\sim \Dc_{\Xc}$ and $y_t= f_t(\x_t)+z$ where $z\sim\Dc_Z$. Here $\Dc_{\Xc}$ is a distribution over $\Xc$ and $\Dc_Z$ is a zero-mean distribution with subgaussian norm bounded by $\sigma$. 
%\end{definition}
%
%
%
%\noindent\textbf{Training the transformer model:} With the setup above, transformer model corresponds to searching for the optimal $\bal\in\Ac$ through empirical risk minimization (ERM) over $\Sca$ as follows.

%Concretely, 

%\smallskip
%\noindent\textbf{Evaluating the transformer model:} We evaluate a transformer model through two closely-related criteria. 
%\begin{itemize}
%\item \textbf{Multitask learning:} The population risk over training contexts $1$ to $T$: $\Lc_{\Dca}(\bal)=\E[\hat{\Lc}_{\Sca}(\bal)]$.
%\item \textbf{Transfer learning:} The population risk over the new task, namely $\Lc_{\Dcn}(\bal)=\E[\hat{\Lc}_{\Scn}(\bal)]$ where
%\[
%\hat{\Lc}_{\Scn}(\bal):=\frac{1}{n-n_0}\sum_{i=n_0+1}^n \ell(\yt{\new}_i,{\bal_{\Sn{\new,i}}(\xt{\new}_i)}).
%\]
%\end{itemize}



==> sec/table_diff.tex <==

\begin{wraptable}{r}{0.50\textwidth}

\centering
\footnotesize{
\begin{tabular}{ |c|c|c| } 
     \hline
      & Vanilla MTL & In-context learning \\ 
     \hline
     Shared across & Representation & Meta ML algorithm \\ 
     \hline
     Task-specific & Classifier head & Prompt \\ 
     \hline
\end{tabular}}\vspace{-5pt}
\caption{\small{Viewing ICL through multitask learning (MTL) highlights a clear parallelism of shared and task-specific components of the learning process.}}
\end{wraptable}
% setting we consider is inherently a meta-learningStatistical analysis of ICL 
